Pose-Aware Self-Supervised Learning with Viewpoint Trajectory Regularization

Learning visual features from unlabeled images has proven successful for semantic categorization, often by mapping different $views$ of the same object to the same feature to achieve recognition invariance. However, visual recognition involves not only identifying $what$ an object is but also understanding $how$ it is presented. For example, seeing a car from the side versus head-on is crucial for deciding whether to stay put or jump out of the way. While unsupervised feature learning for downstream viewpoint reasoning is important, it remains under-explored, partly due to the lack of a standardized evaluation method and benchmarks. We introduce a new dataset of adjacent image triplets obtained from a viewpoint trajectory, without any semantic or pose labels. We benchmark both semantic classification and pose estimation accuracies on the same visual feature. Additionally, we propose a viewpoint trajectory regularization loss for learning features from unlabeled image triplets. Our experiments demonstrate that this approach helps develop a visual representation that encodes object identity and organizes objects by their poses, retaining semantic classification accuracy while achieving emergent global pose awareness and better generalization to novel objects. Our dataset and code are available at http://pwang.pw/trajSSL/.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/archived.tex <==
\begin{table*}[htb]
\centering
\label{tab:feats}
\small{
\resizebox{\linewidth}{!}{
\begin{tabular}{@{} l   @{\hskip 0.03in} | @{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l|@{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l}
\toprule

\multirow{2}{*}{\textbf{Acc. (\%)}} & \multicolumn{2}{c}{\textbf{in-domain}}             & \multicolumn{3}{c}{\textbf{out-of-domain many-shot}} & \multicolumn{2}{c}{\textbf{out-of-domain few-shot}}  \\

                                    & \textbf{semantic clas.} & 
                                    \textbf{exact pose} &\textbf{relative pose} & \textbf{unseen pose}      & \textbf{unseen categories}     & \textbf{unseen pose} & \textbf{unseen categories} \\
 \midrule
\textbf{supervised}                 & 86.4   & 92.2                & 86.11                    & 61.31                     & 77.38                          & 74.05                  & 19.75                      \\  \midrule

\textbf{vicreg}                     & 82.02    &   84.3            & 76.69                    & 59.6                      & 73.05                          & 63.58                  & 62.95                      \\
\textbf{vicreg+traj}                & 82.03   &     87.8          & 80.48                    & 62.68                     & 77.52                          & 57.99                  & 68.75                      \\
\textbf{vicreg+sup. pose}           & 81.57 &  89.8                & 83.77                    & 61.36                     & 77.67                          & 66.34                  & 64.58                      \\  \midrule

\textbf{simclr}                     & 83.36  & 84.8                & 77.28                    & 58.13                     & 68.53                          & 52.56                  &    63.43                     \\
\textbf{simclr+traj}                & 83.40  &   86.4               & 79.47                     & 61.28                     & 71.01                          & 56.05       & 66.75   \\
\bottomrule
\end{tabular}
}
}
\vspace{-6pt}
\caption{Performance at feature layer. \rev{one digit decimal}}
\vspace{-10pt}
\end{table*}

\begin{table}[htb]
\centering
\label{tab:feats}
\small{
\resizebox{\linewidth}{!}{
%\begin{tabular}{@{} l   @{\hskip 0.03in} | @{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l|@{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l}
\begin{tabular}{@{} l | lll|lll|lll}
\toprule

\textbf{Rel. Pose Acc. (\%)}         & \multicolumn{3}{c|}{\textbf{in-domain}} & \multicolumn{3}{c|}{\textbf{unseen pose}} & \multicolumn{3}{c}{\textbf{unseen cat.}} \\   \cmidrule{1-1}

\textbf{embedding}        & conv3       & conv4       & feat       & conv3        & conv4        & feat       & conv3        & conv4        & feat       \\
\midrule
\textbf{supervised}       & 90.5        & 89.0       & 86.1       & 81.6         & 79.3         & 61.3       & 88.0         & 85.6         & 77.4       \\
\midrule
\textbf{vicreg}           & 88.0        & 87.0        & 76.7       & 80.1         & 78.3         & 59.6       & 85.7         & 83.7         & 73.1       \\
\textbf{vicreg+traj}      & {\bf 89.4}        & 88.3        & 80.5       & 82.6         & 80.3         & 62.7       & 88.2         & 85.5         & 77.5       \\
\textbf{vicreg+sup. pose} & 88.8        & 88.9        & 83.8       & 82.7         & 79.6         & 61.4       & 87.7         & 86.1         & 77.6     \\
\bottomrule
\end{tabular}
}
}
\vspace{-6pt}
\caption{Performance at different layer.}
\vspace{-10pt}
\end{table}

\begin{figure*}[htb]
    \centering
   \includegraphics[width=2\columnwidth]{pics/mnist_vis.png}
    \caption{Rotating MNIST (single trajectory).}
    \label{fig:combo1}
      \vspace{-1.5em}
\end{figure*}

TABLE 3 4

\begin{table}[t!]
    \centering
    % First table in the left minipage
    \begin{minipage}[t]{0.48\textwidth}
        \centering
\caption{The proposed trajectory loss $\mathcal{L}_{\text{traj}}$ leads to pose estimation gain without harming semantic classification accuracy. 
Specifically, SSL achieves comparable or marginally superior results than supervised methods for out-of-domain and real data.
%SSL outperforms fully-supervised methods for out-of-domain pose estimation. Compared with geometry-supervised methods (where pose labels are available in training), SSL outperforms them on out-of-domain unseen pose estimation, and is on-part for estimating object pose of unseen semantic classes.
Feature-layer representation $z$ is used for both semantic classification and pose estimation.
%Se at feature layer. 
}

\small{
\resizebox{\linewidth}{!}{
%\begin{tabular}{@{} l   @{\hskip 0.03in} | @{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l|@{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l}
\begin{tabular}{@{} l | lll|ll |l}
\toprule

\multirow{2}{*}{\textbf{Acc. (\%)}} & \multicolumn{3}{c|}{\textbf{in-domain}}             & \multicolumn{2}{c|}{\textbf{out-of-domain pose est.}} &\multicolumn{1}{c}{{\bf real photos}} \\

                                    & \textbf{sem. cls.} & 
                                    \textbf{abs. pose} &\textbf{rel. pose} & \textbf{unseen pose}      & \textbf{unseen sem.} &{\bf cars \cite{shaler2017carvana}  }   \\
 \midrule
  %\multicolumn{6}{l}{\textcolor{gray}{{\it Fully-supervised methods for upper bound}} } \\
\textbf{Fully-Sup. \footnote{\scriptsize We train two separate supervised models for semantic classification and pose estimation, as a supervised multi-task model yields worse results than specialized, separate models.}}                 & {\bf 86.4}   &  {\bf 92.2}                & {\bf 86.1}                    & 61.3                     & 77.4    &      88.5                                          \\
 % \multicolumn{6}{l}{\textcolor{gray}{{\it A geometry-supervised method with pose labels but not semantic labels during training}} } \\

{\bf Geometry-Sup.} %\textbf{vicreg+sup. pose} 
& 85.4 &  89.8                &  83.8                    & 61.4                     & {\bf 77.6}                    &     87.9                     \\
\midrule
  \multicolumn{6}{l}{\textcolor{gray}{{\it Fully-unsupervised methods}} } \\

\textbf{VICRreg \cite{bardes2021vicreg}}                     & 85.6    &   84.3            & 76.7                    & 59.6                      & 73.1       &     88.7                                              \\
\textbf{VICRreg+traj.}                & 85.6   &     87.8\textcolor{red}{($\uparrow$3.5)}      & 80.5\textcolor{red}{($\uparrow$3.8)}                    & {\bf 62.7}\textcolor{red}{($\uparrow$3.1)}                     & {\bf 77.5}\textcolor{red}{($\uparrow$4.4)}     &         {\bf 91.7 }\textcolor{red}{($\uparrow$3.0)}                                 \\
\addlinespace[0.4em]

\textbf{SimCLR \cite{chen2020simple}}                     &  85.9  & 84.8                & 77.3                    & 58.1                    & 68.5                  &     89.0                                    \\
\textbf{SimCLR+traj.}                &  86.0  &   86.4\textcolor{red}{($\uparrow$1.6)}                & 79.5\textcolor{red}{($\uparrow$2.2)}                     & 61.3\textcolor{red}{($\uparrow$3.2)}                      & 71.0\textcolor{red}{($\uparrow$2.5)}           &       91.5\textcolor{red}{($\uparrow$2.5)}     \\
\addlinespace[0.4em]

\textbf{SimSiam \cite{chen2021exploring}}                     &  85.4  & 84.9                & 77.4                    & 57.8                    & 68.1                  &     88.8                                    \\
\textbf{SimSiam+traj.}                &  85.5  &   87.2\textcolor{red}{($\uparrow$2.3)}                & 79.5\textcolor{red}{($\uparrow$2.1)}                     & 61.0\textcolor{red}{($\uparrow$3.2)}                      & 70.8\textcolor{red}{($\uparrow$2.7)}           &       91.2\textcolor{red}{($\uparrow$2.4)}     \\


\bottomrule
\end{tabular}
}
}
        
        \label{tab:feats}
    \end{minipage}
    \hfill % This will insert a space between the two tables
    % Second table in the right minipage
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \vspace{5em}
        \caption{Using mid-layer ``conv3'' rather than last-layer ``feature''
        for relative-pose-estimation downstream task improves accuracy: 9\% for in-domain data and 20\% for out-of-domain unseen poses.
}

\small{
\resizebox{\linewidth}{!}{
%\begin{tabular}{@{} l   @{\hskip 0.03in} | @{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l|@{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l| @{\hskip 0.05in} l}
\begin{tabular}{@{} l | lll|lll|lll}
\toprule

      & \multicolumn{3}{c|}{\textbf{in-domain}} & \multicolumn{3}{c|}{\textbf{unseen pose}} & \multicolumn{3}{c}{\textbf{unseen cat.}} \\   

\textbf{Representation layer}        & conv3       & conv4       & feat       & conv3        & conv4        & feat       & conv3        & conv4        & feat       \\

\midrule
\textbf{Fully-Sup.}       & {\bf 90.5}        & 89.0       & 86.1       & 81.6         & 79.3         & 61.3       & 88.0         & 85.6         & 77.4       \\
\textbf{Geometry-Sup.} & 88.8        & 88.9        & 83.8       & 82.7         & 79.6         & 61.4       & 87.7         & 86.1         & 77.6     \\
\midrule
\textbf{VICReg \cite{bardes2021vicreg}}           & 88.0        & 87.0        & 76.7       & 80.1         & 78.3         & 59.6       & 85.7         & 83.7         & 73.1       \\
\textbf{VICReg+traj.}      &  89.4\textcolor{red}{($\uparrow$9)}        & 88.3        & 80.5       & {\bf 82.6}\textcolor{red}{($\uparrow$20)}         & 80.3         & 62.7       & {\bf 88.2}\textcolor{red}{($\uparrow$11)}         & 85.5         & 77.5       \\

\bottomrule
\multicolumn{1}{l}{Metric: pose acc. (\%)}
\end{tabular}
}
}
        \label{tab:mid}
    \end{minipage}
    \vspace{-1em}
\end{table}


\begin{figure}[t!]
%\vspace{-0.5em}
    \centering
        \begin{minipage}[t!]{0.53\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/teaser.pdf} % Replace 'example-image' with your image file
    \end{minipage}%
    \hfill
    \begin{minipage}[t!]{0.44\textwidth}
        \caption{ We study the geometric and semantic representation quality of self-supervised learning (SSL). {\bf Left:} The model, trained exclusively on images of rotating objects, is assessed for its ability to recover the pose and semantic category of an image. {\bf Right:} Our approach improves pose estimation accuracy by encouraging images with similar poses to form smooth trajectories in the representation space.% and improves pose estimation accuracy.    
}
        \label{fig:image1}
    \end{minipage}
    \vspace{-2em}
    \label{fig:teaser}
\end{figure}

  \begin{table}[t!]
   % \begin{minipage}[t]{0.51\textwidth}
        \centering
        \caption{
        In-domain and out-of-domain split of our benchmark dataset.
        For semantics, we use non-overlapping 13 semantic categories as in-domain and 11 as out-of-domain data. For pose, we render distinct Fib$(50)$ and Fib$(100)$ for each object as in-domain and out-of-domain poses. Only 13 in-domain categories with Fib$(50)$ poses are used for training, while others are for out-of-domain evaluation (visualizations in Fig.\ref{fig:fib}).}
\small{
\resizebox{0.43\linewidth}{!}{
\begin{tabular}{ll|l|l}
\toprule
\multicolumn{2}{l|}{\multirow{2}{*}{ \diagbox[width=12em,height=2.5em]{{\bf Pose}}{{\bf Semantic}} }}       & \textbf{in-domain}   & \textbf{out-of-domain}     \\ 
\multicolumn{2}{l|}{}                                           & 13 classes  & 11 classes        \\ \midrule
\multicolumn{1}{l}{\textbf{in-domain}}     & Fib$(50)$  & 260k     & 220k         \\ 
\multicolumn{1}{l}{\textbf{out-of-domain}} & Fib$(100)$ & 520k  & 440k  \\ 

\bottomrule
\end{tabular}
}
}
        \label{tab:dataset}
  %  \end{minipage}
    \vspace{-0.5em}
\end{table}


\begin{figure}[t!]
    % First figure
    \begin{minipage}[t]{0.515\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/relpose.pdf} % Replace with your first image file
        \caption{{\bf Left:} We adopt {\it absolute} and {\it relative} pose estimation as geometric evaluations. Notably, relative pose enables SSL's generalizability test on out-of-domain data as it eliminates the need for category-specific canonical pose. The (camera) pose is defined as the spherical coordinate (azimuth, elevation) of the camera position. 
        %For an object, we render images with look-at view transforms, which assume the camera is on a unit sphere with up-vector $(0, 1, 0)$ and translation $\vc{t}=(0,0,1)$. The object pose is represented as the (azimuth, elevation) of the camera angle. The figure depicts {\it absolute pose}, where we define a canonical pose for each category. For {\it relative pose}, we take two images with poses $\vc{p_1}, \vc{p_2}$ as inputs, and predict the pose difference $\vc{\Delta p} =\vc{p_2}- \vc{p_1}$.
    {\bf Right:} $(15^{\circ},15^{\circ})$ pose of \textcolor{blue}{in-domain} and \textcolor{red}{out-of-domain} semantic classes, which are plotted with PCA-projected Word2Vec \cite{church2017word2vec}.}
        \label{fig:relpose}
    \end{minipage}
    \hfill % This will insert a space between the two figures
    % Second figure
    \begin{minipage}[t]{0.43\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/fib_v3.pdf} % Replace with your second image file
        \caption{Our benchmark dataset includes renderings of objects from $n$ unique camera angles, uniformly distributed across the viewing sphere $S^2$, utilizing a Fibonacci sphere distribution, denoted as $\text{Fib}(n)$ (upper left shows a case where $n=50$).
    We visualize the non-overlapping split of \textcolor{blue}{in-domain} and \textcolor{red}{out-of-domain} semantic categories and poses.}% The model is trained data with both in-domain poses and semantic categories.}
        \label{fig:fib}
    \end{minipage}
    \vspace{-1.3em}
\end{figure}

\begin{figure}[t!]
    \begin{minipage}{0.35\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/ablation_v2.pdf} % Replace 'example-image' with your image file
    \end{minipage}%
    \hfill
    \begin{minipage}{0.62\textwidth}
        \caption{Hyperparameter analysis on the trajectory-regularized VICReg, which is evaluated for relative pose estimation with representation being the feature-layer $z$. {\bf Upper:} While fixing the feature layer for the downstream task of pose estimation, we change different layers to impose the trajectory loss $\mathcal{L}_{\text{traj}}$. Feature-layer gives the best performance, although the difference is less than 2\%. {\bf Lower:} The highest performance is achieved at trajectory loss weight $\lambda = 0.01$, though the method is not very sensitive to $\lambda$.}
        \vspace{-1.3em}
                \label{fig:ablation}
    \end{minipage}
\end{figure}


\begin{figure}[t!]
    % Left figure
    % Right figure
    \begin{minipage}[t]{0.495\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/net_arch.pdf} % Replace with your right image file
        \caption{In addition to an unsupervised semantic loss $\mathcal{L}_{\text{sem}}$ which is commonly used in SSL, we add a trajectory loss $\mathcal{L}_{\text{traj}}$ (Eqn.\ref{eq:traj})  to enhance geometric representation.
        $\mathcal{L}_{\text{sem}}$ always follows baseline settings, which is applied post-projector for SimCLR, for example. $\mathcal{L}_{\text{traj}}$ always operates on the pooled feature $z$.
        For pose evaluation, we allow representations from different layers and find that mid-layer representations like ``res block3'' give pose estimation gain.
        %We also find mid-layer representations like ``conv3'' lead to pose estimation gain.
        }
        \label{fig:architect}
    \end{minipage}
    \hfill
        \begin{minipage}[t]{0.475\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/linear2.pdf} % Replace with your left image file
        \caption{We enforce representations of adjacent views of an object, $\vc{z_L},\vc{z_C},\vc{z_R}$, to form a geodesic trajectory. {\bf Upper:} $\vc{z}$ resides on a unit hypersphere. The objective is to map the difference vectors $\vc{v_1} = \vc{z_C} - \vc{z_L}$ and $\vc{v_2} = \vc{z_R} - \vc{z_C}$ onto $\vc{z_C}$'s tangent plane, optimizing for maximal cosine similarity to achieve a linear trajectory on that plane. {\bf Lower:} Projected vector $\vc{u}$ is computed by deducting the normal component $\vc{z_C}$ from the  difference vector $\vc{v}$.}
        \label{fig:linear}
    \end{minipage}
    \vspace{-1em}
\end{figure}

\begin{figure}[t!]
\vspace{-1em}
\includegraphics[width=\linewidth]{figure/teaser_v2.pdf} \vspace{-1em}
\caption{Our goal is to capture two aspects of object recognition through SSL: {\it what the object is} and {\it how the object is presented}.
While the former has been well studied \cite{chen2020simple,bardes2021vicreg}, the latter is rarely understood.
We learn SSL representations that not only capture object identity but also pose.
{\bf a)} The training data are image triplets with subtle viewpoint changes of an object. The object identity, semantics and pose are unknown.
{\bf b)} The learned representations are expected to discriminate different object semantics and poses and to achieve high accuracies for both semantic classification and pose estimation. Notably, we expect to understand {\it global pose} from {\it local pose} changes.
%cluster and classify object semantics and pose when projecting to the corresponding axis.
{\bf c)} Our approach improves pose estimation accuracy over existing methods \cite{bardes2021vicreg} by encouraging images with similar poses to form smooth trajectories in the representation space.
}
       % \caption{ {\bf Left:} We consider two pillars of SSL for object recognition: {\it what is the object} and {\it how is it presented}. While the former has been well studied, the latter is rarely understood. In this paper, we study the geometric and semantic representation quality of self-supervised learning (SSL) and propose pose-aware SSL that achieves high accuracies for both semantic classification and pose estimation.  {\bf Middle:} The model, trained exclusively on images of rotating objects, is assessed for its ability to recover the pose and semantic category of an image. {\bf Right:} Our approach improves pose estimation accuracy by encouraging images with similar poses to form smooth trajectories in the representation space.% and improves pose estimation accuracy.  }
        \label{fig:image1}
        \vspace{-1.5em}
\end{figure}


%old intro
 

\vspace{-1.5em}
\section{Introduction}
\label{sec:intro}







%The emergence of self-supervised learning (SSL) of image representation \cite{wu2018unsupervised,chen2020simple,bardes2021vicreg} has marked a significant advancement over  supervised methods. SSL's ability to uncover intrinsic data patterns without reliance on labels offers remarkable flexibility and adaptability to real-world scenarios. A crucial aspect of further enhancing SSL's real-world applicability involves its proficiency in learning both semantic and geometric representations. Despite SSL's success in semantic tasks like classification and detection, its effectiveness in geometric representation learning and the methodologies for its evaluation remain largely unexplored. This study seeks to establish a benchmark for assessing SSL's geometric representation capabilities and introduces methods to bolster this aspect of learning.




The emergence of self-supervised learning (SSL) of image representations has enabled many advantages over its supervised counterparts, such as discovering inherent data patterns without labels \cite{wu2018unsupervised,chen2020simple,bardes2021vicreg}, high flexibility \cite{oquab2023dinov2} and generalizability when adapting to real-world data \cite{pantazis2021focus,wang2022unsupervised}.
More recently, SSL has greatly improved the performance of foundation models, LLMs and VLMs \cite{achiam2023gpt,bai2024sequential}.
% method does not matter much, data matters; useful for data w/o labels
% To further improve SSL's generalizability to real-world data, the ability to learn good semantic and geometric representations is essential. 
However, most SSL methods focus on coarse-grained recognition: They are designed to recognize {\it what the object is}, rather than {\it how the object is presented}. As a result, many state-of-art models suffer poor performance for objects with less common poses, ranging from task-specific \cite{wang2022unsupervised} to foundation models \cite{el2024probing}.
One reason is that such models usually lack training data with a full cover of object poses, which is pivotal for robust performance \cite{schuhmann2022laion,li2024datacomp}.
%many foundation models cannot recognize objects with less common poses \cite{el2024probing}.
Additionally, most SSL is only evaluated on semantic tasks, e.g. classification and detection, and its effectiveness for pose-aware representation learning %geometric representation learning 
remains relatively unexplored \cite{dangovski2021equivariant}.
The absence of a standardized evaluation method for geometric self-supervised representations worsens these issues.
%This is partially due to the absence of a standardized evaluation method for geometric self-supervised representations.
%We establish

This work establishes a new benchmark for assessing SSL's geometric representation capabilities. We also propose methods to enhance the self-supervised geometric representation quality with trajectory regularization of objects with subtle view changes.%, including using mid-level representations and trajectory regularization.% loss.
%introduces a trajectory-regularization loss to enhance the self-supervised geometric representation quality.

%Indeed, our work is not limited to pose estimation. Although it is on pose..., our method can be extended to other geometric tasks (like depth and surface normal other than the pose esitmation, which, by itself is an important question.  (temporal consistency can ) We will add more discussions in the final version.

\begin{figure}[t!]
\vspace{-0.5em}
\includegraphics[width=\linewidth]{figure/teaser_v2.pdf} % Replace 'example-image' with your image file
\vspace{-1em}
\caption{Our goal is to capture two aspects of object recognition through SSL: {\it what the object is} and {\it how the object is presented}.
While the former has been well studied \cite{chen2020simple,bardes2021vicreg}, the latter is rarely understood.
We learn SSL representations that not only capture object identity but also pose.
{\bf a)} The training data are image triplets with subtle pose changes of an object. The object identity, semantics and pose are unknown.
{\bf b)} The learned representations are expected to discriminate different object semantics and poses and to achieve high accuracies for both semantic classification and pose estimation. Notably, we expect to understand {\it global pose} from {\it local pose changes}.
%cluster and classify object semantics and pose when projecting to the corresponding axis.
{\bf c)} Our approach improves pose estimation accuracy over existing methods \cite{bardes2021vicreg} by encouraging images with similar poses to form smooth trajectories in the representation space.
}
       % \caption{ {\bf Left:} We consider two pillars of SSL for object recognition: {\it what is the object} and {\it how is it presented}. While the former has been well studied, the latter is rarely understood. In this paper, we study the geometric and semantic representation quality of self-supervised learning (SSL) and propose pose-aware SSL that achieves high accuracies for both semantic classification and pose estimation.  {\bf Middle:} The model, trained exclusively on images of rotating objects, is assessed for its ability to recover the pose and semantic category of an image. {\bf Right:} Our approach improves pose estimation accuracy by encouraging images with similar poses to form smooth trajectories in the representation space.% and improves pose estimation accuracy.  }
        \label{fig:image1}
        \vspace{-1.5em}
\end{figure}
 



% \begin{table}[htb]
% \caption{\small  Supervised learning relies on labels in training. SSL, which does not rely on ground-truth pose or semantic labels during training, offers improved model flexibility and generalizability. Our SSL  incorporates an unsupervised geometry-trajectory-regularization loss, thereby enhancing geometric representations.
% }
% \centering
% \small{
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|c|c|c}
% \toprule
% {\bf Method} &	{\bf semantic label} &	{\bf pose label} &	{\bf traj. reg.} \\

%  \midrule

% Fully-Supervised \cite{zhang2022relpose,lin2023relpose++} &	\cmark &	\cmark	&\xmark\\
% Geometry-Supervised \cite{dangovski2021equivariant,garrido2023self}	& \xmark &	\cmark	&\xmark \\
% Invariant SSL (baseline) \cite{bardes2021vicreg,chen2020simple}	&\xmark &	\xmark	&\xmark\\
% {\bf Trajectory-Regularized SSL (ours)}	&\xmark &	\xmark	&\cmark\\

% \bottomrule
% \end{tabular}
% }
% }
%     \vspace{-1.5em}

% \label{tab:method_comp}
% \end{table}

%\pw{Rewrite this part to emphasize motivation and benchmark setting + relative pose}

%paragraph 2: setting (robotics). We can boil down to representations that have both semantics and geometry. 

%Learning representation for joint recognition of object semantics and pose could benefit many scenarios such as video analysis \cite{grauman2022ego4d}, robotics \cite{du2021vision} and world-models \cite{sergeant2023influence}.
%However, 
The quality of SSL representations for geometric tasks is relatively underexplored, partially due to the absence of established benchmarks. This work proposes a benchmark that evaluates SSL's performance on both semantic classification and pose estimation for object-centric images, given the benefits of joint recognition of object semantics and pose in scenarios like video analysis \cite{grauman2022ego4d}, robotics \cite{du2021vision} and world-models \cite{sergeant2023influence}.
First, we define a setting where SSL should learn both semantic and geometric representations. %representations for both semantic and geometric downstream tasks. 
Our benchmark precludes the use of semantic or pose labels during training and encompasses both semantic classification and pose estimation downstream tasks during evaluation, unlike existing settings \cite{garrido2023self,lee2021improving} which allow training SSL with pose labels. 
%Our benchmark has two novelties:
Additionally, we enable out-of-domain pose estimation by introducing relative pose estimation. 
Without the necessity of defining category-specific canonical pose, SSL can be flexibly evaluated on out-of-domain data and unseen categories.
Finally, our benchmark provides data generation configurations, leading to 
a dataset containing images of different objects with different poses, which is challenging for both semantic and geometric downstream tasks. Images are also sampled as short sequences with slight camera pose changes. % where the camera slightly moves around the objects. 
The sequence could serve as a natural prior since humans and animals have access to video data instead of i.i.d. samples. 
%Our benchmark dataset contains images of different objects with different pose configurations, where SSLs are evaluated for both pose estimation and semantic classification downstream tasks. %which is challenging for both pose estimation and semantic classification downstream tasks. 
% dataset derived from the ShapeNet \cite{chang2015shapenet} dataset. The dataset
%First: define setting of joint semantic-pose; Second: enable OOD test

%Two insights: 1) patch; 2) trajectory (we choose a simple way)

%(1- single image) 
%(2- squence)


%Our benchmark dataset contains images of different objects with different pose configurations, which is challenging for both pose estimation and semantic classification downstream tasks. 
%Further, the images are sampled as sequences where the camera moves around the objects. The sequence information is provided as a natural prior since humans and animals have access to video data instead of i.i.d. samples. Given a learned representation, we establish metrics to evaluate its performance on both semantic classification and geometric pose estimation. Additionally, we also assess the generalization to out-of-distribution categories and pose tasks. 

Based on the benchmark, we evaluate the geometric representation quality of existing SSL methods. On a ResNet backbone, we discover that using mid-layer representation for pose estimation leads to 10-20\% performance gain compared to the feature from the higher layers, likely owing to its similarity to patch embedding and alignment with mid-level vision tasks. 
Our method is inspired by a natural learning scenario where humans recognize objects with saccades, a rapid eye movement that shifts the gaze from one part of the visual field to another.  
We learn joint representation from many separate sets of adjacent views of different objects \ref{fig:image1} and propose a trajectory regularization method to encourage adjacent frames from the image sequences to form a smooth trajectory in the representation space, inspired by slow feature analysis \cite{foldiak1991learning, wiskott2002slow, goroshin2015learning, chen2018sparse}. 
The trajectory regularization uses a simple local linearity assumption and leads to an additional 4\% improvement for pose estimation without affecting semantic classification. Furthermore, we provide qualitative visualization and quantitative evaluation on a real-world rotating-car dataset Carvana \cite{shaler2017carvana} to further confirm the effectiveness of the proposed method. 


To summarize, our contributions are:
\begin{enumerate} %make it inline! emphasize that we are general, mild representation changes for similar poses
    \item {\bf Introduction of a Novel Benchmark for Geometric SSL Evaluation.}
    We present a new benchmark for evaluating both geometric and semantic representations of self-supervised learning, which defines the  setting and allows evaluations on out-of-domain data. %which precludes the use of semantic or pose labels during training and encompasses both types of tasks during evaluation.%where during training neither semantic nor geometric labels are available and during evaluations both semantic and geometric downstream tasks are considered.

    %\item {\bf Improving Pose Estimation with Mid-Layer Representations.}
    %We find mid-layer representations lead to pose estimation gain (10\%-20\%), partially due to their ability to capture local features like patch embedding. 
    %We compress high-dimensional mid-layer representations, striking a balance between efficiency and performance. .

    \item {\bf Proposal of Unsupervised Trajectory Regularization Loss.}
    We analyze a ResNet trained on the benchmark and observe that representations in earlier convolution blocks have better pose estimation accuracies (10\%-20\%), partially due to their ability to capture local structures like patch embedding. 
    To further improve the representation strictures, we introduce a novel unsupervised trajectory regularization loss that encourages smooth representation trajectories for adjacent views of an object.
    %the representations of different views of an object to form a smooth trajectory in the representation space. 
    It improves pose-estimation performance (4\%).

    %the architecture for geometry-aware representations, and find pose and semantics should be learned separately (the earlier layer is better for pose. and later better for semantics).
\end{enumerate} 

% We use 3D object pose estimation as a downstream task and surrogate for evaluating the geometric representation quality. 
% We adopt a setting for the new benchmark as follows:
% during training, neither ground-truth semantic labels nor pose labels should be used;
% during evaluation, the model should concurrently learn semantic and geometric representations, with the capability for corresponding downstream tasks. 
% %To enable practical implementations, w
% We also provide a benchmark dataset derived from ShapeNet \cite{chang2015shapenet} along with comprehensive training and evaluation protocols.
% The downstream tasks include semantic classification and pose estimation, with the latter performed on both in-domain and out-of-domain images, accompanied by extensive evaluation metrics. Our setting of SSL from multi-category objects with various poses may help applications like 3D reconstruction \cite{wang2023sparsenerf} and robotic grasping \cite{shen2023distilled}.


%The learned representations should contain semantic and pose information of the input.
%Thus, during evaluation, we study performance for both semantic and pose estimation performance, such as NN and probe.
%For the output, the representations should be aware of both semantics and pose.
%Further, we 
%Side: why SIE not working: assume GT pose known.

%Our exploration into methods that enhance geometric representation learning, while preserving semantic integrity, yields notable insights. We observe that leveraging mid-layer representations for pose estimation can improve performance by 10\%-20\%, likely owing to its alignment with mid-level vision tasks. Additionally, we demonstrate that these mid-layer representations can be efficiently compressed, reducing computational overhead without significant loss in performance. Furthermore, we propose a linearization regularization technique for adjacent poses, inspired by slow feature analysis. This approach creates a trajectory in the representation space as the object pose varies, leading to a 4\% improvement in pose estimation accuracy without affecting semantic classification.







%In addition to evaluating state-of-the-art SSL methods on the proposed benchmark, we study two 
% We also study methods that enhance geometric representation learning without hurting semantic representations, based on our evaluation and observation of the state-of-the-art SSL on the proposed benchmark.
% First, we find that using mid-layer representation for pose estimation leads to 10-20\% performance gain, likely owing to its alignment with mid-level vision tasks. We further show that mid-layer representations can be efficiently compressed, reducing computational overhead without significant loss in performance. %which reduces the computation burden from the high dimensionality.
% Secondly, we propose a linearization regularization for adjacent poses, inspired by slow feature analysis \cite{foldiak1991learning, wiskott2002slow, goroshin2015learning, chen2018sparse}.
% This regularization leads to a trajectory in the representation space as the object rotates, leading to an additional 4\% improvement for pose estimation without affecting semantic classification.
%We show that such a prior leads to a trajectory of an object with different poses in the representation space, which improves the pose estimation accuracy by 4\% without compromising the semantic classification performance.

%[contribution 2] Mid-layer.In addition to the invariance prior widely used in SSL, We propose a linearization regularization, which dates back to slow feature analysis, and show such a prior improves the pose representation without compromising the semantic representation.

%[What we do, detailed method explanation]: 1) When the object rotates, we encourage its representation to form a smooth trajectory.Specifically, we encourage local linearization, that is, representations of the object with slightly different poses form a linear trajectory. %how we construct the input and linear trajectory loss;
%2) Further, we find that using the latent embedding from earlier layers as pose representation leads to better pose estimation performance.  While earlier-layer representations have higher dimensions, we show that they can be compressed with limited performance loss.
%We also show  earlier-layer representations, which usually are of high dimension, can be efficiently compressed with limited performance loss.
%1) we evaluate baseline SSL methods and their representations can be used for pose estimation;  2) we leverage a natural prior for learning and propose a new loss. 3) we evaluate different layers as representations for evaluating semantics and geometry;




